MONAA: A Tool for Timed Pattern Matching with Automata-Based Acceleration

We present monaa, a monitoring tool over a real-time property specified by either a timed automaton or a timed regular expression. It implements a timed pattern matching algorithm that combines 1) features suited for online monitoring, and 2) acceleration by automata-based skipping. Our experiments demonstrate monaa's performance advantage, especially in online usage.

==> figs/0128050447/plotMonaaTime.tex <==
\begin{tikzpicture}[gnuplot]
%% generated with GNUPLOT 5.2p2 (Lua 5.3; terminal rev. 99, script rev. 102)
%% Wed Jan 31 15:19:50 2018
\path (0.000,0.000) rectangle (12.500,8.750);
\gpcolor{color=gp lt color border}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\gpsetlinewidth{1.00}
\draw[gp path] (1.320,0.985)--(1.500,0.985);
\draw[gp path] (11.947,0.985)--(11.767,0.985);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (1.136,0.985) {$0$};
\draw[gp path] (1.320,2.228)--(1.500,2.228);
\draw[gp path] (11.947,2.228)--(11.767,2.228);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (1.136,2.228) {$50$};
\draw[gp path] (1.320,3.470)--(1.500,3.470);
\draw[gp path] (11.947,3.470)--(11.767,3.470);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (1.136,3.470) {$100$};
\draw[gp path] (1.320,4.713)--(1.500,4.713);
\draw[gp path] (11.947,4.713)--(11.767,4.713);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (1.136,4.713) {$150$};
\draw[gp path] (1.320,5.956)--(1.500,5.956);
\draw[gp path] (11.947,5.956)--(11.767,5.956);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (1.136,5.956) {$200$};
\draw[gp path] (1.320,7.198)--(1.500,7.198);
\draw[gp path] (11.947,7.198)--(11.767,7.198);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (1.136,7.198) {$250$};
\draw[gp path] (1.320,8.441)--(1.500,8.441);
\draw[gp path] (11.947,8.441)--(11.767,8.441);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (1.136,8.441) {$300$};
\draw[gp path] (1.320,0.985)--(1.320,1.165);
\draw[gp path] (1.320,8.441)--(1.320,8.261);
\node[gp node center,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (1.320,0.677) {$0$};
\draw[gp path] (3.091,0.985)--(3.091,1.165);
\draw[gp path] (3.091,8.441)--(3.091,8.261);
\node[gp node center,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (3.091,0.677) {$2$};
\draw[gp path] (4.862,0.985)--(4.862,1.165);
\draw[gp path] (4.862,8.441)--(4.862,8.261);
\node[gp node center,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (4.862,0.677) {$4$};
\draw[gp path] (6.634,0.985)--(6.634,1.165);
\draw[gp path] (6.634,8.441)--(6.634,8.261);
\node[gp node center,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (6.634,0.677) {$6$};
\draw[gp path] (8.405,0.985)--(8.405,1.165);
\draw[gp path] (8.405,8.441)--(8.405,8.261);
\node[gp node center,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (8.405,0.677) {$8$};
\draw[gp path] (10.176,0.985)--(10.176,1.165);
\draw[gp path] (10.176,8.441)--(10.176,8.261);
\node[gp node center,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (10.176,0.677) {$10$};
\draw[gp path] (11.947,0.985)--(11.947,1.165);
\draw[gp path] (11.947,8.441)--(11.947,8.261);
\node[gp node center,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (11.947,0.677) {$12$};
\draw[gp path] (1.320,8.441)--(1.320,0.985)--(11.947,0.985)--(11.947,8.441)--cycle;
\node[gp node center,rotate=-270,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (0.276,4.713) {Execution Time [sec.]};
\node[gp node center,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (6.633,0.215) {Length of Timed Words [$\times 100000$]};
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (9.927,8.030) {MONAA (TRE)};
\gpcolor{rgb color={0.580,0.000,0.827}}
\draw[gp path] (10.203,8.030)--(11.487,8.030);
\draw[gp path] (1.323,2.956)--(2.450,2.959)--(3.585,2.987)--(4.713,2.985)--(5.825,3.017)%
  --(6.921,3.140)--(8.037,3.051)--(9.243,3.063)--(10.277,3.064);
\gpsetpointsize{4.00}
\gppoint{gp mark 1}{(1.323,2.956)}
\gppoint{gp mark 1}{(2.450,2.959)}
\gppoint{gp mark 1}{(3.585,2.987)}
\gppoint{gp mark 1}{(4.713,2.985)}
\gppoint{gp mark 1}{(5.825,3.017)}
\gppoint{gp mark 1}{(6.921,3.140)}
\gppoint{gp mark 1}{(8.037,3.051)}
\gppoint{gp mark 1}{(9.243,3.063)}
\gppoint{gp mark 1}{(10.277,3.064)}
\gppoint{gp mark 1}{(10.845,8.030)}
\gpcolor{color=gp lt color border}
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (9.927,7.568) {MONAA (TA)};
\gpcolor{rgb color={0.000,0.620,0.451}}
\draw[gp path] (10.203,7.568)--(11.487,7.568);
\draw[gp path] (1.323,0.990)--(2.450,0.993)--(3.585,0.995)--(4.713,0.998)--(5.825,1.001)%
  --(6.921,1.004)--(8.037,1.006)--(9.243,1.009)--(10.277,1.012);
\gppoint{gp mark 2}{(1.323,0.990)}
\gppoint{gp mark 2}{(2.450,0.993)}
\gppoint{gp mark 2}{(3.585,0.995)}
\gppoint{gp mark 2}{(4.713,0.998)}
\gppoint{gp mark 2}{(5.825,1.001)}
\gppoint{gp mark 2}{(6.921,1.004)}
\gppoint{gp mark 2}{(8.037,1.006)}
\gppoint{gp mark 2}{(9.243,1.009)}
\gppoint{gp mark 2}{(10.277,1.012)}
\gppoint{gp mark 2}{(10.845,7.568)}
\gpcolor{color=gp lt color border}
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (9.927,7.106) {libmonaa hard-coded autom.};
\gpcolor{rgb color={0.337,0.706,0.914}}
\draw[gp path] (10.203,7.106)--(11.487,7.106);
\draw[gp path] (1.323,0.988)--(2.450,1.806)--(3.585,2.568)--(4.713,3.335)--(5.825,4.252)%
  --(6.921,4.964)--(8.037,5.775)--(9.243,6.699)--(10.277,7.456);
\gppoint{gp mark 3}{(1.323,0.988)}
\gppoint{gp mark 3}{(2.450,1.806)}
\gppoint{gp mark 3}{(3.585,2.568)}
\gppoint{gp mark 3}{(4.713,3.335)}
\gppoint{gp mark 3}{(5.825,4.252)}
\gppoint{gp mark 3}{(6.921,4.964)}
\gppoint{gp mark 3}{(8.037,5.775)}
\gppoint{gp mark 3}{(9.243,6.699)}
\gppoint{gp mark 3}{(10.277,7.456)}
\gppoint{gp mark 3}{(10.845,7.106)}
\gpcolor{color=gp lt color border}
\draw[gp path] (1.320,8.441)--(1.320,0.985)--(11.947,0.985)--(11.947,8.441)--cycle;
%% coordinates of the plot area
\gpdefrectangularnode{gp plot 1}{\pgfpoint{1.320cm}{0.985cm}}{\pgfpoint{11.947cm}{8.441cm}}
\end{tikzpicture}
%% gnuplot variables


==> figs/0129053206/plotMonaaTime.tex <==
\begin{tikzpicture}[gnuplot]
%% generated with GNUPLOT 5.2p2 (Lua 5.3; terminal rev. 99, script rev. 102)
%% Wed Jan 31 15:19:50 2018
\path (0.000,0.000) rectangle (12.500,8.750);
\gpcolor{color=gp lt color border}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\gpsetlinewidth{1.00}
\draw[gp path] (1.320,0.985)--(1.500,0.985);
\draw[gp path] (11.947,0.985)--(11.767,0.985);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (1.136,0.985) {$0$};
\draw[gp path] (1.320,1.731)--(1.500,1.731);
\draw[gp path] (11.947,1.731)--(11.767,1.731);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (1.136,1.731) {$0.5$};
\draw[gp path] (1.320,2.476)--(1.500,2.476);
\draw[gp path] (11.947,2.476)--(11.767,2.476);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (1.136,2.476) {$1$};
\draw[gp path] (1.320,3.222)--(1.500,3.222);
\draw[gp path] (11.947,3.222)--(11.767,3.222);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (1.136,3.222) {$1.5$};
\draw[gp path] (1.320,3.967)--(1.500,3.967);
\draw[gp path] (11.947,3.967)--(11.767,3.967);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (1.136,3.967) {$2$};
\draw[gp path] (1.320,4.713)--(1.500,4.713);
\draw[gp path] (11.947,4.713)--(11.767,4.713);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (1.136,4.713) {$2.5$};
\draw[gp path] (1.320,5.459)--(1.500,5.459);
\draw[gp path] (11.947,5.459)--(11.767,5.459);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (1.136,5.459) {$3$};
\draw[gp path] (1.320,6.204)--(1.500,6.204);
\draw[gp path] (11.947,6.204)--(11.767,6.204);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (1.136,6.204) {$3.5$};
\draw[gp path] (1.320,6.950)--(1.500,6.950);
\draw[gp path] (11.947,6.950)--(11.767,6.950);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (1.136,6.950) {$4$};
\draw[gp path] (1.320,7.695)--(1.500,7.695);
\draw[gp path] (11.947,7.695)--(11.767,7.695);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (1.136,7.695) {$4.5$};
\draw[gp path] (1.320,8.441)--(1.500,8.441);
\draw[gp path] (11.947,8.441)--(11.767,8.441);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (1.136,8.441) {$5$};
\draw[gp path] (1.320,0.985)--(1.320,1.165);
\draw[gp path] (1.320,8.441)--(1.320,8.261);
\node[gp node center,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (1.320,0.677) {$0$};
\draw[gp path] (3.091,0.985)--(3.091,1.165);
\draw[gp path] (3.091,8.441)--(3.091,8.261);
\node[gp node center,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (3.091,0.677) {$2$};
\draw[gp path] (4.862,0.985)--(4.862,1.165);
\draw[gp path] (4.862,8.441)--(4.862,8.261);
\node[gp node center,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (4.862,0.677) {$4$};
\draw[gp path] (6.634,0.985)--(6.634,1.165);
\draw[gp path] (6.634,8.441)--(6.634,8.261);
\node[gp node center,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (6.634,0.677) {$6$};
\draw[gp path] (8.405,0.985)--(8.405,1.165);
\draw[gp path] (8.405,8.441)--(8.405,8.261);
\node[gp node center,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (8.405,0.677) {$8$};
\draw[gp path] (10.176,0.985)--(10.176,1.165);
\draw[gp path] (10.176,8.441)--(10.176,8.261);
\node[gp node center,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (10.176,0.677) {$10$};
\draw[gp path] (11.947,0.985)--(11.947,1.165);
\draw[gp path] (11.947,8.441)--(11.947,8.261);
\node[gp node center,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (11.947,0.677) {$12$};
\draw[gp path] (1.320,8.441)--(1.320,0.985)--(11.947,0.985)--(11.947,8.441)--cycle;
\node[gp node center,rotate=-270,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (0.276,4.713) {Execution Time [sec.]};
\node[gp node center,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (6.633,0.215) {Length of Timed Words [$\times 100000$]};
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (9.927,8.030) {MONAA (TRE)};
\gpcolor{rgb color={0.580,0.000,0.827}}
\draw[gp path] (10.203,8.030)--(11.487,8.030);
\draw[gp path] (1.323,1.224)--(2.450,1.134)--(3.585,1.134)--(4.713,1.134)--(5.825,1.134)%
  --(6.921,1.134)--(8.037,1.134)--(9.243,1.134)--(10.277,1.134);
\gpsetpointsize{4.00}
\gppoint{gp mark 1}{(1.323,1.224)}
\gppoint{gp mark 1}{(2.450,1.134)}
\gppoint{gp mark 1}{(3.585,1.134)}
\gppoint{gp mark 1}{(4.713,1.134)}
\gppoint{gp mark 1}{(5.825,1.134)}
\gppoint{gp mark 1}{(6.921,1.134)}
\gppoint{gp mark 1}{(8.037,1.134)}
\gppoint{gp mark 1}{(9.243,1.134)}
\gppoint{gp mark 1}{(10.277,1.134)}
\gppoint{gp mark 1}{(10.845,8.030)}
\gpcolor{color=gp lt color border}
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (9.927,7.568) {MONAA (TA)};
\gpcolor{rgb color={0.000,0.620,0.451}}
\draw[gp path] (10.203,7.568)--(11.487,7.568);
\draw[gp path] (1.323,2.208)--(2.450,2.879)--(3.585,3.580)--(4.713,4.355)--(5.825,4.981)%
  --(6.921,5.682)--(8.037,6.398)--(9.243,7.084)--(10.277,7.785);
\gppoint{gp mark 2}{(1.323,2.208)}
\gppoint{gp mark 2}{(2.450,2.879)}
\gppoint{gp mark 2}{(3.585,3.580)}
\gppoint{gp mark 2}{(4.713,4.355)}
\gppoint{gp mark 2}{(5.825,4.981)}
\gppoint{gp mark 2}{(6.921,5.682)}
\gppoint{gp mark 2}{(8.037,6.398)}
\gppoint{gp mark 2}{(9.243,7.084)}
\gppoint{gp mark 2}{(10.277,7.785)}
\gppoint{gp mark 2}{(10.845,7.568)}
\gpcolor{color=gp lt color border}
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (9.927,7.106) {libmonaa hard-coded autom.};
\gpcolor{rgb color={0.337,0.706,0.914}}
\draw[gp path] (10.203,7.106)--(11.487,7.106);
\draw[gp path] (1.323,1.298)--(2.450,1.447)--(3.585,1.611)--(4.713,1.775)--(5.825,1.939)%
  --(6.921,2.103)--(8.037,2.267)--(9.243,2.431)--(10.277,2.595);
\gppoint{gp mark 3}{(1.323,1.298)}
\gppoint{gp mark 3}{(2.450,1.447)}
\gppoint{gp mark 3}{(3.585,1.611)}
\gppoint{gp mark 3}{(4.713,1.775)}
\gppoint{gp mark 3}{(5.825,1.939)}
\gppoint{gp mark 3}{(6.921,2.103)}
\gppoint{gp mark 3}{(8.037,2.267)}
\gppoint{gp mark 3}{(9.243,2.431)}
\gppoint{gp mark 3}{(10.277,2.595)}
\gppoint{gp mark 3}{(10.845,7.106)}
\gpcolor{color=gp lt color border}
\draw[gp path] (1.320,8.441)--(1.320,0.985)--(11.947,0.985)--(11.947,8.441)--cycle;
%% coordinates of the plot area
\gpdefrectangularnode{gp plot 1}{\pgfpoint{1.320cm}{0.985cm}}{\pgfpoint{11.947cm}{8.441cm}}
\end{tikzpicture}
%% gnuplot variables


==> figs/0129072214/plotMonaaTime.tex <==
\begin{tikzpicture}[gnuplot]
%% generated with GNUPLOT 5.2p2 (Lua 5.3; terminal rev. 99, script rev. 102)
%% Wed Jan 31 15:19:50 2018
\path (0.000,0.000) rectangle (12.500,8.750);
\gpcolor{color=gp lt color border}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\gpsetlinewidth{1.00}
\draw[gp path] (1.136,0.985)--(1.316,0.985);
\draw[gp path] (11.947,0.985)--(11.767,0.985);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (0.952,0.985) {$0$};
\draw[gp path] (1.136,1.917)--(1.316,1.917);
\draw[gp path] (11.947,1.917)--(11.767,1.917);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (0.952,1.917) {$2$};
\draw[gp path] (1.136,2.849)--(1.316,2.849);
\draw[gp path] (11.947,2.849)--(11.767,2.849);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (0.952,2.849) {$4$};
\draw[gp path] (1.136,3.781)--(1.316,3.781);
\draw[gp path] (11.947,3.781)--(11.767,3.781);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (0.952,3.781) {$6$};
\draw[gp path] (1.136,4.713)--(1.316,4.713);
\draw[gp path] (11.947,4.713)--(11.767,4.713);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (0.952,4.713) {$8$};
\draw[gp path] (1.136,5.645)--(1.316,5.645);
\draw[gp path] (11.947,5.645)--(11.767,5.645);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (0.952,5.645) {$10$};
\draw[gp path] (1.136,6.577)--(1.316,6.577);
\draw[gp path] (11.947,6.577)--(11.767,6.577);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (0.952,6.577) {$12$};
\draw[gp path] (1.136,7.509)--(1.316,7.509);
\draw[gp path] (11.947,7.509)--(11.767,7.509);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (0.952,7.509) {$14$};
\draw[gp path] (1.136,8.441)--(1.316,8.441);
\draw[gp path] (11.947,8.441)--(11.767,8.441);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (0.952,8.441) {$16$};
\draw[gp path] (1.136,0.985)--(1.136,1.165);
\draw[gp path] (1.136,8.441)--(1.136,8.261);
\node[gp node center,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (1.136,0.677) {$0$};
\draw[gp path] (2.938,0.985)--(2.938,1.165);
\draw[gp path] (2.938,8.441)--(2.938,8.261);
\node[gp node center,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (2.938,0.677) {$2$};
\draw[gp path] (4.740,0.985)--(4.740,1.165);
\draw[gp path] (4.740,8.441)--(4.740,8.261);
\node[gp node center,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (4.740,0.677) {$4$};
\draw[gp path] (6.542,0.985)--(6.542,1.165);
\draw[gp path] (6.542,8.441)--(6.542,8.261);
\node[gp node center,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (6.542,0.677) {$6$};
\draw[gp path] (8.343,0.985)--(8.343,1.165);
\draw[gp path] (8.343,8.441)--(8.343,8.261);
\node[gp node center,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (8.343,0.677) {$8$};
\draw[gp path] (10.145,0.985)--(10.145,1.165);
\draw[gp path] (10.145,8.441)--(10.145,8.261);
\node[gp node center,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (10.145,0.677) {$10$};
\draw[gp path] (11.947,0.985)--(11.947,1.165);
\draw[gp path] (11.947,8.441)--(11.947,8.261);
\node[gp node center,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (11.947,0.677) {$12$};
\draw[gp path] (1.136,8.441)--(1.136,0.985)--(11.947,0.985)--(11.947,8.441)--cycle;
\node[gp node center,rotate=-270,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (0.276,4.713) {Execution Time [sec.]};
\node[gp node center,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (6.541,0.215) {Length of Timed Words [$\times 100000$]};
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (9.927,8.030) {MONAA (TRE)};
\gpcolor{rgb color={0.580,0.000,0.827}}
\draw[gp path] (10.203,8.030)--(11.487,8.030);
\draw[gp path] (1.139,6.349)--(2.285,6.656)--(3.440,6.950)--(4.588,7.048)--(5.719,7.733)%
  --(6.834,7.691)--(7.969,7.756)--(9.196,8.003)--(10.248,8.269);
\gpsetpointsize{4.00}
\gppoint{gp mark 1}{(1.139,6.349)}
\gppoint{gp mark 1}{(2.285,6.656)}
\gppoint{gp mark 1}{(3.440,6.950)}
\gppoint{gp mark 1}{(4.588,7.048)}
\gppoint{gp mark 1}{(5.719,7.733)}
\gppoint{gp mark 1}{(6.834,7.691)}
\gppoint{gp mark 1}{(7.969,7.756)}
\gppoint{gp mark 1}{(9.196,8.003)}
\gppoint{gp mark 1}{(10.248,8.269)}
\gppoint{gp mark 1}{(10.845,8.030)}
\gpcolor{color=gp lt color border}
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (9.927,7.568) {MONAA (TA)};
\gpcolor{rgb color={0.000,0.620,0.451}}
\draw[gp path] (10.203,7.568)--(11.487,7.568);
\draw[gp path] (1.139,1.362)--(2.285,1.581)--(3.440,1.796)--(4.588,2.015)--(5.719,2.239)%
  --(6.834,2.490)--(7.969,2.746)--(9.196,2.896)--(10.248,3.129);
\gppoint{gp mark 2}{(1.139,1.362)}
\gppoint{gp mark 2}{(2.285,1.581)}
\gppoint{gp mark 2}{(3.440,1.796)}
\gppoint{gp mark 2}{(4.588,2.015)}
\gppoint{gp mark 2}{(5.719,2.239)}
\gppoint{gp mark 2}{(6.834,2.490)}
\gppoint{gp mark 2}{(7.969,2.746)}
\gppoint{gp mark 2}{(9.196,2.896)}
\gppoint{gp mark 2}{(10.248,3.129)}
\gppoint{gp mark 2}{(10.845,7.568)}
\gpcolor{color=gp lt color border}
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (9.927,7.106) {libmonaa hard-coded autom.};
\gpcolor{rgb color={0.337,0.706,0.914}}
\draw[gp path] (10.203,7.106)--(11.487,7.106);
\draw[gp path] (1.139,1.083)--(2.285,1.129)--(3.440,1.181)--(4.588,1.232)--(5.719,1.283)%
  --(6.834,1.335)--(7.969,1.386)--(9.196,1.437)--(10.248,1.488);
\gppoint{gp mark 3}{(1.139,1.083)}
\gppoint{gp mark 3}{(2.285,1.129)}
\gppoint{gp mark 3}{(3.440,1.181)}
\gppoint{gp mark 3}{(4.588,1.232)}
\gppoint{gp mark 3}{(5.719,1.283)}
\gppoint{gp mark 3}{(6.834,1.335)}
\gppoint{gp mark 3}{(7.969,1.386)}
\gppoint{gp mark 3}{(9.196,1.437)}
\gppoint{gp mark 3}{(10.248,1.488)}
\gppoint{gp mark 3}{(10.845,7.106)}
\gpcolor{color=gp lt color border}
\draw[gp path] (1.136,8.441)--(1.136,0.985)--(11.947,0.985)--(11.947,8.441)--cycle;
%% coordinates of the plot area
\gpdefrectangularnode{gp plot 1}{\pgfpoint{1.136cm}{0.985cm}}{\pgfpoint{11.947cm}{8.441cm}}
\end{tikzpicture}
%% gnuplot variables


==> figs/0129094951/plotMonaaTime.tex <==
\begin{tikzpicture}[gnuplot]
%% generated with GNUPLOT 5.2p2 (Lua 5.3; terminal rev. 99, script rev. 102)
%% Wed Jan 31 15:19:50 2018
\path (0.000,0.000) rectangle (12.500,8.750);
\gpcolor{color=gp lt color border}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\gpsetlinewidth{1.00}
\draw[gp path] (1.136,0.985)--(1.316,0.985);
\draw[gp path] (11.947,0.985)--(11.767,0.985);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (0.952,0.985) {$0$};
\draw[gp path] (1.136,2.228)--(1.316,2.228);
\draw[gp path] (11.947,2.228)--(11.767,2.228);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (0.952,2.228) {$2$};
\draw[gp path] (1.136,3.470)--(1.316,3.470);
\draw[gp path] (11.947,3.470)--(11.767,3.470);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (0.952,3.470) {$4$};
\draw[gp path] (1.136,4.713)--(1.316,4.713);
\draw[gp path] (11.947,4.713)--(11.767,4.713);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (0.952,4.713) {$6$};
\draw[gp path] (1.136,5.956)--(1.316,5.956);
\draw[gp path] (11.947,5.956)--(11.767,5.956);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (0.952,5.956) {$8$};
\draw[gp path] (1.136,7.198)--(1.316,7.198);
\draw[gp path] (11.947,7.198)--(11.767,7.198);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (0.952,7.198) {$10$};
\draw[gp path] (1.136,8.441)--(1.316,8.441);
\draw[gp path] (11.947,8.441)--(11.767,8.441);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (0.952,8.441) {$12$};
\draw[gp path] (1.136,0.985)--(1.136,1.165);
\draw[gp path] (1.136,8.441)--(1.136,8.261);
\node[gp node center,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (1.136,0.677) {$0$};
\draw[gp path] (2.938,0.985)--(2.938,1.165);
\draw[gp path] (2.938,8.441)--(2.938,8.261);
\node[gp node center,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (2.938,0.677) {$2$};
\draw[gp path] (4.740,0.985)--(4.740,1.165);
\draw[gp path] (4.740,8.441)--(4.740,8.261);
\node[gp node center,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (4.740,0.677) {$4$};
\draw[gp path] (6.542,0.985)--(6.542,1.165);
\draw[gp path] (6.542,8.441)--(6.542,8.261);
\node[gp node center,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (6.542,0.677) {$6$};
\draw[gp path] (8.343,0.985)--(8.343,1.165);
\draw[gp path] (8.343,8.441)--(8.343,8.261);
\node[gp node center,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (8.343,0.677) {$8$};
\draw[gp path] (10.145,0.985)--(10.145,1.165);
\draw[gp path] (10.145,8.441)--(10.145,8.261);
\node[gp node center,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (10.145,0.677) {$10$};
\draw[gp path] (11.947,0.985)--(11.947,1.165);
\draw[gp path] (11.947,8.441)--(11.947,8.261);
\node[gp node center,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (11.947,0.677) {$12$};
\draw[gp path] (1.136,8.441)--(1.136,0.985)--(11.947,0.985)--(11.947,8.441)--cycle;
\node[gp node center,rotate=-270,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (0.276,4.713) {Execution Time [sec.]};
\node[gp node center,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (6.541,0.215) {Length of Timed Words [$\times 100000$]};
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (9.927,8.030) {MONAA (TRE)};
\gpcolor{rgb color={0.580,0.000,0.827}}
\draw[gp path] (10.203,8.030)--(11.487,8.030);
\draw[gp path] (1.139,5.353)--(2.285,5.676)--(3.440,5.987)--(4.588,6.291)--(5.719,6.676)%
  --(6.834,6.906)--(7.969,7.229)--(9.196,7.528)--(10.248,7.851);
\gpsetpointsize{4.00}
\gppoint{gp mark 1}{(1.139,5.353)}
\gppoint{gp mark 1}{(2.285,5.676)}
\gppoint{gp mark 1}{(3.440,5.987)}
\gppoint{gp mark 1}{(4.588,6.291)}
\gppoint{gp mark 1}{(5.719,6.676)}
\gppoint{gp mark 1}{(6.834,6.906)}
\gppoint{gp mark 1}{(7.969,7.229)}
\gppoint{gp mark 1}{(9.196,7.528)}
\gppoint{gp mark 1}{(10.248,7.851)}
\gppoint{gp mark 1}{(10.845,8.030)}
\gpcolor{color=gp lt color border}
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (9.927,7.568) {MONAA (TA)};
\gpcolor{rgb color={0.000,0.620,0.451}}
\draw[gp path] (10.203,7.568)--(11.487,7.568);
\draw[gp path] (1.139,1.482)--(2.285,1.774)--(3.440,2.060)--(4.588,2.358)--(5.719,2.656)%
  --(6.834,2.936)--(7.969,3.222)--(9.196,3.508)--(10.248,3.818);
\gppoint{gp mark 2}{(1.139,1.482)}
\gppoint{gp mark 2}{(2.285,1.774)}
\gppoint{gp mark 2}{(3.440,2.060)}
\gppoint{gp mark 2}{(4.588,2.358)}
\gppoint{gp mark 2}{(5.719,2.656)}
\gppoint{gp mark 2}{(6.834,2.936)}
\gppoint{gp mark 2}{(7.969,3.222)}
\gppoint{gp mark 2}{(9.196,3.508)}
\gppoint{gp mark 2}{(10.248,3.818)}
\gppoint{gp mark 2}{(10.845,7.568)}
\gpcolor{color=gp lt color border}
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (9.927,7.106) {libmonaa hard-coded autom.};
\gpcolor{rgb color={0.337,0.706,0.914}}
\draw[gp path] (10.203,7.106)--(11.487,7.106);
\draw[gp path] (1.139,1.109)--(2.285,1.178)--(3.440,1.246)--(4.588,1.314)--(5.719,1.383)%
  --(6.834,1.451)--(7.969,1.513)--(9.196,1.588)--(10.248,1.650);
\gppoint{gp mark 3}{(1.139,1.109)}
\gppoint{gp mark 3}{(2.285,1.178)}
\gppoint{gp mark 3}{(3.440,1.246)}
\gppoint{gp mark 3}{(4.588,1.314)}
\gppoint{gp mark 3}{(5.719,1.383)}
\gppoint{gp mark 3}{(6.834,1.451)}
\gppoint{gp mark 3}{(7.969,1.513)}
\gppoint{gp mark 3}{(9.196,1.588)}
\gppoint{gp mark 3}{(10.248,1.650)}
\gppoint{gp mark 3}{(10.845,7.106)}
\gpcolor{color=gp lt color border}
\draw[gp path] (1.136,8.441)--(1.136,0.985)--(11.947,0.985)--(11.947,8.441)--cycle;
%% coordinates of the plot area
\gpdefrectangularnode{gp plot 1}{\pgfpoint{1.136cm}{0.985cm}}{\pgfpoint{11.947cm}{8.441cm}}
\end{tikzpicture}
%% gnuplot variables


==> figs/gnuplot-lua-tikz-common.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%     Common style file for TeX, LaTeX and ConTeXt
%%  
%%  It is associated with the 'gnuplot.lua' script, and usually generated
%%  automatically. So take care whenever you make any changes!
%%

% check for the correct TikZ version
\def\gpchecktikzversion#1.#2\relax{%
\ifnum#1<2%
  \errmessage{PGF/TikZ version >= 2.0 is required!}%
\fi}
\expandafter\gpchecktikzversion\pgfversion\relax

% FIXME: is there a more elegant way to determine the output format?

\def\pgfsysdriver@a{pgfsys-dvi.def}       % ps
\def\pgfsysdriver@b{pgfsys-dvipdfm.def}   % pdf
\def\pgfsysdriver@c{pgfsys-dvipdfmx.def}  % pdf
\def\pgfsysdriver@d{pgfsys-dvips.def}     % ps
\def\pgfsysdriver@e{pgfsys-pdftex.def}    % pdf
\def\pgfsysdriver@f{pgfsys-tex4ht.def}    % html
\def\pgfsysdriver@g{pgfsys-textures.def}  % ps
\def\pgfsysdriver@h{pgfsys-vtex.def}      % ps
\def\pgfsysdriver@i{pgfsys-xetex.def}     % pdf

\newif\ifgppdfout\gppdfoutfalse
\newif\ifgppsout\gppsoutfalse

\ifx\pgfsysdriver\pgfsysdriver@a
  \gppsouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@b
  \gppdfouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@c
  \gppdfouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@d
  \gppsouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@e
  \gppdfouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@f
  % tex4ht
\else\ifx\pgfsysdriver\pgfsysdriver@g
  \gppsouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@h
  \gppsouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@i
  \gppdfouttrue
\fi\fi\fi\fi\fi\fi\fi\fi\fi

% uncomment the following lines to make font values "appendable"
% and if you are really sure about that ;-)
% \pgfkeyslet{/tikz/font/.@cmd}{\undefined}
% \tikzset{font/.initial={}}
% \def\tikz@textfont{\pgfkeysvalueof{/tikz/font}}

%
% image related stuff
%
\def\gp@rawimage@pdf#1#2#3#4#5#6{%
  \def\gp@tempa{cmyk}%
  \def\gp@tempb{#1}%
  \ifx\gp@tempa\gp@tempb%
    \def\gp@temp{/CMYK}%
  \else%
    \def\gp@temp{/RGB}%
  \fi%
  \pgf@sys@bp{#4}\pgfsysprotocol@literalbuffered{0 0}\pgf@sys@bp{#5}%
  \pgfsysprotocol@literalbuffered{0 0 cm}%
  \pgfsysprotocol@literalbuffered{BI /W #2 /H #3 /CS \gp@temp}%
  \pgfsysprotocol@literalbuffered{/BPC 8 /F /AHx ID}%
  \pgfsysprotocol@literal{#6 > EI}%
}
\def\gp@rawimage@ps#1#2#3#4#5#6{%
  \def\gp@tempa{cmyk}%
  \def\gp@tempb{#1}%
  \ifx\gp@tempa\gp@tempb%
    \def\gp@temp{4}%
  \else%
    \def\gp@temp{3}%
  \fi%
  \pgfsysprotocol@literalbuffered{0 0 translate}%
  \pgf@sys@bp{#4}\pgf@sys@bp{#5}\pgfsysprotocol@literalbuffered{scale}%
  \pgfsysprotocol@literalbuffered{#2 #3 8 [#2 0 0 -#3 0 #3]}%
  \pgfsysprotocol@literalbuffered{currentfile /ASCIIHexDecode filter}%
  \pgfsysprotocol@literalbuffered{false \gp@temp\space colorimage}%
  \pgfsysprotocol@literal{#6 >}%
}
\def\gp@rawimage@html#1#2#3#4#5#6{%
% FIXME: print a warning message here
}

\ifgppdfout
  \def\gp@rawimage{\gp@rawimage@pdf}
\else
  \ifgppsout
    \def\gp@rawimage{\gp@rawimage@ps}
  \else
    \def\gp@rawimage{\gp@rawimage@html}
  \fi
\fi


\def\gploadimage#1#2#3#4#5{%
  \pgftext[left,bottom,x=#1cm,y=#2cm] {\pgfimage[interpolate=false,width=#3cm,height=#4cm]{#5}};%
}

\def\gp@set@size#1{%
  \def\gp@image@size{#1}%
}

\def\gp@rawimage@#1#2#3#4#5#6#7#8{
  \tikz@scan@one@point\gp@set@size(#6,#7)\relax%
  \tikz@scan@one@point\pgftransformshift(#2,#3)\relax%
  \pgftext {%
    \pgfsys@beginpurepicture%
    \gp@image@size% fill \pgf@x and \pgf@y
    \gp@rawimage{#1}{#4}{#5}{\pgf@x}{\pgf@y}{#8}%
    \pgfsys@endpurepicture%
  }%
}

%% \gprawimage{color model}{xcoord}{ycoord}{# of xpixel}{# of ypixel}{xsize}{ysize}{rgb/cmyk hex data RRGGBB/CCMMYYKK ...}{file name}
%% color model is 'cmyk' or 'rgb' (default)
\def\gprawimage#1#2#3#4#5#6#7#8#9{%
  \ifx&#9&%
    \gp@rawimage@{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}
  \else
    \ifgppsout
      \gp@rawimage@{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}
    \else
      \gploadimage{#2}{#3}{#6}{#7}{#9}
    \fi
  \fi
}

%
% gnuplottex comapatibility
% (see http://www.ctan.org/tex-archive/help/Catalogue/entries/gnuplottex.html)
%

\def\gnuplottexextension@lua{\string tex}
\def\gnuplottexextension@tikz{\string tex}

%
% gnuplot variables getter and setter
%

\def\gpsetvar#1#2{%
  \expandafter\xdef\csname gp@var@#1\endcsname{#2}
}

\def\gpgetvar#1{%
  \csname gp@var@#1\endcsname %
}

%
% some wrapper code
%

% short for a filled path
\def\gpfill#1{\path[line width=0.1\gpbaselw,draw,fill,#1]}

% short for changing the line width
\def\gpsetlinewidth#1{\pgfsetlinewidth{#1\gpbaselw}}

% short for changing the line type
\def\gpsetlinetype#1{\tikzset{gp path/.style={#1,#1 add}}}

% short for changing the dash pattern
\def\gpsetdashtype#1{\tikzset{gp path/.append style={#1}}}

% short for changing the point size
\def\gpsetpointsize#1{\tikzset{gp point/.style={mark size=#1\gpbasems}}}

% wrapper for color settings
\def\gpcolor#1{\tikzset{global #1}}
\tikzset{rgb color/.code={\pgfutil@definecolor{.}{rgb}{#1}\tikzset{color=.}}}
\tikzset{global rgb color/.code={\pgfutil@definecolor{.}{rgb}{#1}\pgfutil@color{.}}}
\tikzset{global color/.code={\pgfutil@color{#1}}}

% prevent plot mark distortions due to changes in the PGF transformation matrix
% use `\gpscalepointstrue' and `\gpscalepointsfalse' for enabling and disabling
% point scaling
%
\newif\ifgpscalepoints
\tikzset{gp shift only/.style={%
  \ifgpscalepoints\else shift only\fi%
}}
\def\gppoint#1#2{%
  \path[solid] plot[only marks,gp point,mark options={gp shift only},#1] coordinates {#2};%
}


%
% char size calculation, that might be used with gnuplottex
%
% Example code (needs gnuplottex.sty):
%
%    % calculate the char size when the "gnuplot" style is used
%    \tikzset{gnuplot/.append style={execute at begin picture=\gpcalccharsize}}
%
%    \tikzset{gnuplot/.append style={font=\ttfamily\footnotesize}}
%
%    \begin{tikzpicture}[gnuplot]
%      \begin{gnuplot}[terminal=lua,%
%          terminaloptions={tikz solid nopic charsize \the\gphcharsize,\the\gpvcharsize}]
%        test
%      \end{gnuplot}
%    \end{tikzpicture}
%
%%%
% The `\gpcalccharsize' command fills the lengths \gpvcharsize and \gphcharsize with
% the values of the current default font used within nodes and is meant to be called
% within a tikzpicture environment.
% 
\newdimen\gpvcharsize
\newdimen\gphcharsize
\def\gpcalccharsize{%
  \pgfinterruptboundingbox%
  \pgfsys@begininvisible%
  \node at (0,0) {%
    \global\gphcharsize=1.05\fontcharwd\font`0%
    \global\gpvcharsize=1.05\fontcharht\font`0%
    \global\advance\gpvcharsize by 1.05\fontchardp\font`g%
  };%
  \pgfsys@endinvisible%
  \endpgfinterruptboundingbox%
}

%
%  define a rectangular node in tikz e.g. for the plot area
%
%  #1 node name
%  #2 coordinate of "south west"
%  #3 coordinate of "north east"
%
\def\gpdefrectangularnode#1#2#3{%
  \expandafter\gdef\csname pgf@sh@ns@#1\endcsname{rectangle}
  \expandafter\gdef\csname pgf@sh@np@#1\endcsname{%
    \def\southwest{#2}%
    \def\northeast{#3}%
  }
  \pgfgettransform\pgf@temp%
  % once it is defined, no more transformations will be applied, I hope
  \expandafter\xdef\csname pgf@sh@nt@#1\endcsname{\pgf@temp}%
  \expandafter\xdef\csname pgf@sh@pi@#1\endcsname{\pgfpictureid}%
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%  You may want to adapt the following to fit your needs (in your 
%%  individual style file and/or within your document).
%%

%
% style for every plot
%
\tikzset{gnuplot/.style={%
  >=stealth',%
  line cap=round,%
  line join=round,%
}}

\tikzset{gp node left/.style={anchor=mid west,yshift=-.12ex}}
\tikzset{gp node center/.style={anchor=mid,yshift=-.12ex}}
\tikzset{gp node right/.style={anchor=mid east,yshift=-.12ex}}

% basic plot mark size (points)
\newdimen\gpbasems
\gpbasems=.4pt

% basic linewidth
\newdimen\gpbaselw
\gpbaselw=.4pt

% this is the default color for pattern backgrounds
\colorlet{gpbgfillcolor}{white}

% set background color and fill color
\def\gpsetbgcolor#1{%
  \pgfutil@definecolor{gpbgfillcolor}{rgb}{#1}%
  \tikzset{tight background,background rectangle/.style={fill=gpbgfillcolor},show background rectangle}%
}

% this should reverse the normal text node presets, for the
% later referencing as described below
\tikzset{gp refnode/.style={coordinate,yshift=.12ex}}

% to add an empty label with the referenceable name "my node"
% to the plot, just add the following line to your gnuplot
% file:
%
% set label "" at 1,1 font ",gp refnode,name=my node"
%

% enlargement of the bounding box in standalone mode (only used by LaTeX/ConTeXt)
\def\gpbboxborder{0mm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%  The following TikZ-styles are derived from the 'pgf.styles.*' tables
%%  in the Lua script.
%%  To change the number of used styles you should change them there and
%%  regenerate this style file.
%%

% arrow styles settings
\tikzset{gp arrow 1/.style={>=latex}}
\tikzset{gp arrow 2/.style={>=angle 90}}
\tikzset{gp arrow 3/.style={>=angle 60}}
\tikzset{gp arrow 4/.style={>=angle 45}}
\tikzset{gp arrow 5/.style={>=o}}
\tikzset{gp arrow 6/.style={>=*}}
\tikzset{gp arrow 7/.style={>=diamond}}
\tikzset{gp arrow 8/.style={>=open diamond}}
\tikzset{gp arrow 9/.style={>={]}}}
\tikzset{gp arrow 10/.style={>={[}}}
\tikzset{gp arrow 11/.style={>=)}}
\tikzset{gp arrow 12/.style={>=(}}

% plotmark settings
\tikzset{gp mark 0/.style={mark size=.5\pgflinewidth,mark=*}}
\tikzset{gp mark 1/.style={mark=+}}
\tikzset{gp mark 2/.style={mark=x}}
\tikzset{gp mark 3/.style={mark=star}}
\tikzset{gp mark 4/.style={mark=square}}
\tikzset{gp mark 5/.style={mark=square*}}
\tikzset{gp mark 6/.style={mark=o}}
\tikzset{gp mark 7/.style={mark=*}}
\tikzset{gp mark 8/.style={mark=triangle}}
\tikzset{gp mark 9/.style={mark=triangle*}}
\tikzset{gp mark 10/.style={mark=triangle,every mark/.append style={rotate=180}}}
\tikzset{gp mark 11/.style={mark=triangle*,every mark/.append style={rotate=180}}}
\tikzset{gp mark 12/.style={mark=diamond}}
\tikzset{gp mark 13/.style={mark=diamond*}}
\tikzset{gp mark 14/.style={mark=otimes}}
\tikzset{gp mark 15/.style={mark=oplus}}

% pattern settings
\tikzset{gp pattern 0/.style={white}}
\tikzset{gp pattern 1/.style={pattern=north east lines}}
\tikzset{gp pattern 2/.style={pattern=north west lines}}
\tikzset{gp pattern 3/.style={pattern=crosshatch}}
\tikzset{gp pattern 4/.style={pattern=grid}}
\tikzset{gp pattern 5/.style={pattern=vertical lines}}
\tikzset{gp pattern 6/.style={pattern=horizontal lines}}
\tikzset{gp pattern 7/.style={pattern=dots}}
\tikzset{gp pattern 8/.style={pattern=crosshatch dots}}
\tikzset{gp pattern 9/.style={pattern=fivepointed stars}}
\tikzset{gp pattern 10/.style={pattern=sixpointed stars}}
\tikzset{gp pattern 11/.style={pattern=bricks}}

% if the 'tikzplot' option is used the corresponding lines will be smoothed by default
\tikzset{gp plot axes/.style=}
\tikzset{gp plot border/.style=}
\tikzset{gp plot 0/.style=smooth}
\tikzset{gp plot 1/.style=smooth}
\tikzset{gp plot 2/.style=smooth}
\tikzset{gp plot 3/.style=smooth}
\tikzset{gp plot 4/.style=smooth}
\tikzset{gp plot 5/.style=smooth}
\tikzset{gp plot 6/.style=smooth}
\tikzset{gp plot 7/.style=smooth}

% linestyle settings
\tikzset{gp lt axes/.style=dotted}
\tikzset{gp lt border/.style=solid}

% linestyle "addon" settings for overwriting a default linestyle within the
% TeX document via eg. \tikzset{gp lt plot 1 add/.style={fill=black,draw=none}} etc.
\tikzset{gp lt axes add/.style={}}
\tikzset{gp lt border add/.style={}}
\tikzset{gp lt plot 0 add/.style={}}
\tikzset{gp lt plot 1 add/.style={}}
\tikzset{gp lt plot 2 add/.style={}}
\tikzset{gp lt plot 3 add/.style={}}
\tikzset{gp lt plot 4 add/.style={}}
\tikzset{gp lt plot 5 add/.style={}}
\tikzset{gp lt plot 6 add/.style={}}
\tikzset{gp lt plot 7 add/.style={}}
\tikzset{gp lt plot 0/.style={}}
\tikzset{gp lt plot 1/.style={}}
\tikzset{gp lt plot 2/.style={}}
\tikzset{gp lt plot 3/.style={}}
\tikzset{gp lt plot 4/.style={}}
\tikzset{gp lt plot 5/.style={}}
\tikzset{gp lt plot 6/.style={}}
\tikzset{gp lt plot 7/.style={}}

% linestyle color settings
\colorlet{gp lt color axes}{black!30}
\colorlet{gp lt color border}{black}

% dash type settings
% Define this as a macro so that the dash patterns expand later with the current \pgflinewidth.
\def\gpdashlength{\pgflinewidth}
\tikzset{gp dt 0/.style={solid}}
\tikzset{gp dt 1/.style={solid}}
\tikzset{gp dt 2/.style={dash pattern=on 7.5*\gpdashlength off 7.5*\gpdashlength}}
\tikzset{gp dt 3/.style={dash pattern=on 3.75*\gpdashlength off 5.625*\gpdashlength}}
\tikzset{gp dt 4/.style={dash pattern=on 1*\gpdashlength off 2.8125*\gpdashlength}}
\tikzset{gp dt 5/.style={dash pattern=on 11.25*\gpdashlength off 3.75*\gpdashlength on 1*\gpdashlength off 3.75*\gpdashlength}}
\tikzset{gp dt 6/.style={dash pattern=on 5.625*\gpdashlength off 5.625*\gpdashlength on 1*\gpdashlength off 5.625*\gpdashlength}}
\tikzset{gp dt 7/.style={dash pattern=on 3.75*\gpdashlength off 3.75*\gpdashlength on 3.75*\gpdashlength off 11.25*\gpdashlength}}
\tikzset{gp dt 8/.style={dash pattern=on 1*\gpdashlength off 3.75*\gpdashlength on 11.25*\gpdashlength off 3.75*\gpdashlength on 1*\gpdashlength off 3.75*\gpdashlength}}
\tikzset{gp dt solid/.style={solid}}
\tikzset{gp dt axes/.style={dotted}}

% command for switching to colored lines
\def\gpcoloredlines{%
  \colorlet{gp lt color 0}{red}%
  \colorlet{gp lt color 1}{green}%
  \colorlet{gp lt color 2}{blue}%
  \colorlet{gp lt color 3}{magenta}%
  \colorlet{gp lt color 4}{cyan}%
  \colorlet{gp lt color 5}{yellow}%
  \colorlet{gp lt color 6}{orange}%
  \colorlet{gp lt color 7}{purple}%
}

% command for switching to monochrome (black) lines
\def\gpmonochromelines{%
  \colorlet{gp lt color 0}{black}%
  \colorlet{gp lt color 1}{black}%
  \colorlet{gp lt color 2}{black}%
  \colorlet{gp lt color 3}{black}%
  \colorlet{gp lt color 4}{black}%
  \colorlet{gp lt color 5}{black}%
  \colorlet{gp lt color 6}{black}%
  \colorlet{gp lt color 7}{black}%
}

%
% some initialisations
%
% by default all lines will be colored
\gpcoloredlines
\gpsetpointsize{4}
\gpsetlinetype{gp lt solid}
\gpscalepointsfalse
\endinput


==> figs/plotMonaaTime.tex <==
\begin{tikzpicture}[gnuplot]
%% generated with GNUPLOT 5.2p4 (Lua 5.3; terminal rev. 99 , script rev. 105)
%% Thu Jun  7 18:36:25 2018
\path (0.000,0.000) rectangle (12.500,8.750);
\gpcolor{color=gp lt color border}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\gpsetlinewidth{1.00}
\draw[gp path] (1.320,0.985)--(1.500,0.985);
\draw[gp path] (11.947,0.985)--(11.767,0.985);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (1.136,0.985) {$0$};
\draw[gp path] (1.320,2.050)--(1.500,2.050);
\draw[gp path] (11.947,2.050)--(11.767,2.050);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (1.136,2.050) {$0.2$};
\draw[gp path] (1.320,3.115)--(1.500,3.115);
\draw[gp path] (11.947,3.115)--(11.767,3.115);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (1.136,3.115) {$0.4$};
\draw[gp path] (1.320,4.180)--(1.500,4.180);
\draw[gp path] (11.947,4.180)--(11.767,4.180);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (1.136,4.180) {$0.6$};
\draw[gp path] (1.320,5.246)--(1.500,5.246);
\draw[gp path] (11.947,5.246)--(11.767,5.246);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (1.136,5.246) {$0.8$};
\draw[gp path] (1.320,6.311)--(1.500,6.311);
\draw[gp path] (11.947,6.311)--(11.767,6.311);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (1.136,6.311) {$1$};
\draw[gp path] (1.320,7.376)--(1.500,7.376);
\draw[gp path] (11.947,7.376)--(11.767,7.376);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (1.136,7.376) {$1.2$};
\draw[gp path] (1.320,8.441)--(1.500,8.441);
\draw[gp path] (11.947,8.441)--(11.767,8.441);
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (1.136,8.441) {$1.4$};
\draw[gp path] (1.320,0.985)--(1.320,1.165);
\draw[gp path] (1.320,8.441)--(1.320,8.261);
\node[gp node center,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (1.320,0.677) {$0$};
\draw[gp path] (3.091,0.985)--(3.091,1.165);
\draw[gp path] (3.091,8.441)--(3.091,8.261);
\node[gp node center,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (3.091,0.677) {$200000$};
\draw[gp path] (4.862,0.985)--(4.862,1.165);
\draw[gp path] (4.862,8.441)--(4.862,8.261);
\node[gp node center,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (4.862,0.677) {$400000$};
\draw[gp path] (6.634,0.985)--(6.634,1.165);
\draw[gp path] (6.634,8.441)--(6.634,8.261);
\node[gp node center,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (6.634,0.677) {$600000$};
\draw[gp path] (8.405,0.985)--(8.405,1.165);
\draw[gp path] (8.405,8.441)--(8.405,8.261);
\node[gp node center,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (8.405,0.677) {$800000$};
\draw[gp path] (10.176,0.985)--(10.176,1.165);
\draw[gp path] (10.176,8.441)--(10.176,8.261);
\node[gp node center,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (10.176,0.677) {$1\times10^{6}$};
\draw[gp path] (11.947,0.985)--(11.947,1.165);
\draw[gp path] (11.947,8.441)--(11.947,8.261);
\node[gp node center,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (11.947,0.677) {$1.2\times10^{6}$};
\draw[gp path] (1.320,8.441)--(1.320,0.985)--(11.947,0.985)--(11.947,8.441)--cycle;
\node[gp node center,rotate=-270,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (0.276,4.713) {Execution Time [sec.]};
\node[gp node center,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (6.633,0.215) {Length of Timed Words};
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (9.927,8.030) {MONAA};
\gpcolor{rgb color={0.580,0.000,0.827}}
\draw[gp path] (10.203,8.030)--(11.487,8.030);
\draw[gp path] (1.323,1.251)--(2.450,1.944)--(3.585,2.902)--(4.713,3.808)--(5.825,4.713)%
  --(6.921,5.618)--(8.037,6.524)--(9.243,7.589)--(10.277,8.334);
\gpsetpointsize{4.00}
\gppoint{gp mark 1}{(1.323,1.251)}
\gppoint{gp mark 1}{(2.450,1.944)}
\gppoint{gp mark 1}{(3.585,2.902)}
\gppoint{gp mark 1}{(4.713,3.808)}
\gppoint{gp mark 1}{(5.825,4.713)}
\gppoint{gp mark 1}{(6.921,5.618)}
\gppoint{gp mark 1}{(8.037,6.524)}
\gppoint{gp mark 1}{(9.243,7.589)}
\gppoint{gp mark 1}{(10.277,8.334)}
\gppoint{gp mark 1}{(10.845,8.030)}
\gpcolor{color=gp lt color border}
\node[gp node right,font={\fontsize{15.0pt}{18.0pt}\selectfont}] at (9.927,7.568) {libmonaa hard-coded autom.};
\gpcolor{rgb color={0.000,0.620,0.451}}
\draw[gp path] (10.203,7.568)--(11.487,7.568);
\draw[gp path] (1.323,0.985)--(2.450,1.198)--(3.585,1.358)--(4.713,1.571)--(5.825,1.731)%
  --(6.921,1.944)--(8.037,2.157)--(9.243,2.316)--(10.277,2.529);
\gppoint{gp mark 2}{(1.323,0.985)}
\gppoint{gp mark 2}{(2.450,1.198)}
\gppoint{gp mark 2}{(3.585,1.358)}
\gppoint{gp mark 2}{(4.713,1.571)}
\gppoint{gp mark 2}{(5.825,1.731)}
\gppoint{gp mark 2}{(6.921,1.944)}
\gppoint{gp mark 2}{(8.037,2.157)}
\gppoint{gp mark 2}{(9.243,2.316)}
\gppoint{gp mark 2}{(10.277,2.529)}
\gppoint{gp mark 2}{(10.845,7.568)}
\gpcolor{color=gp lt color border}
\draw[gp path] (1.320,8.441)--(1.320,0.985)--(11.947,0.985)--(11.947,8.441)--cycle;
%% coordinates of the plot area
\gpdefrectangularnode{gp plot 1}{\pgfpoint{1.320cm}{0.985cm}}{\pgfpoint{11.947cm}{8.441cm}}
\end{tikzpicture}
%% gnuplot variables


==> gnuplot-lua-tikz-common.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%     Common style file for TeX, LaTeX and ConTeXt
%%  
%%  It is associated with the 'gnuplot.lua' script, and usually generated
%%  automatically. So take care whenever you make any changes!
%%

% check for the correct TikZ version
\def\gpchecktikzversion#1.#2\relax{%
\ifnum#1<2%
  \errmessage{PGF/TikZ version >= 2.0 is required!}%
\fi}
\expandafter\gpchecktikzversion\pgfversion\relax

% FIXME: is there a more elegant way to determine the output format?

\def\pgfsysdriver@a{pgfsys-dvi.def}       % ps
\def\pgfsysdriver@b{pgfsys-dvipdfm.def}   % pdf
\def\pgfsysdriver@c{pgfsys-dvipdfmx.def}  % pdf
\def\pgfsysdriver@d{pgfsys-dvips.def}     % ps
\def\pgfsysdriver@e{pgfsys-pdftex.def}    % pdf
\def\pgfsysdriver@f{pgfsys-tex4ht.def}    % html
\def\pgfsysdriver@g{pgfsys-textures.def}  % ps
\def\pgfsysdriver@h{pgfsys-vtex.def}      % ps
\def\pgfsysdriver@i{pgfsys-xetex.def}     % pdf

\newif\ifgppdfout\gppdfoutfalse
\newif\ifgppsout\gppsoutfalse

\ifx\pgfsysdriver\pgfsysdriver@a
  \gppsouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@b
  \gppdfouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@c
  \gppdfouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@d
  \gppsouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@e
  \gppdfouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@f
  % tex4ht
\else\ifx\pgfsysdriver\pgfsysdriver@g
  \gppsouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@h
  \gppsouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@i
  \gppdfouttrue
\fi\fi\fi\fi\fi\fi\fi\fi\fi

% uncomment the following lines to make font values "appendable"
% and if you are really sure about that ;-)
% \pgfkeyslet{/tikz/font/.@cmd}{\undefined}
% \tikzset{font/.initial={}}
% \def\tikz@textfont{\pgfkeysvalueof{/tikz/font}}

%
% image related stuff
%
\def\gp@rawimage@pdf#1#2#3#4#5#6{%
  \def\gp@tempa{cmyk}%
  \def\gp@tempb{#1}%
  \ifx\gp@tempa\gp@tempb%
    \def\gp@temp{/CMYK}%
  \else%
    \def\gp@temp{/RGB}%
  \fi%
  \pgf@sys@bp{#4}\pgfsysprotocol@literalbuffered{0 0}\pgf@sys@bp{#5}%
  \pgfsysprotocol@literalbuffered{0 0 cm}%
  \pgfsysprotocol@literalbuffered{BI /W #2 /H #3 /CS \gp@temp}%
  \pgfsysprotocol@literalbuffered{/BPC 8 /F /AHx ID}%
  \pgfsysprotocol@literal{#6 > EI}%
}
\def\gp@rawimage@ps#1#2#3#4#5#6{%
  \def\gp@tempa{cmyk}%
  \def\gp@tempb{#1}%
  \ifx\gp@tempa\gp@tempb%
    \def\gp@temp{4}%
  \else%
    \def\gp@temp{3}%
  \fi%
  \pgfsysprotocol@literalbuffered{0 0 translate}%
  \pgf@sys@bp{#4}\pgf@sys@bp{#5}\pgfsysprotocol@literalbuffered{scale}%
  \pgfsysprotocol@literalbuffered{#2 #3 8 [#2 0 0 -#3 0 #3]}%
  \pgfsysprotocol@literalbuffered{currentfile /ASCIIHexDecode filter}%
  \pgfsysprotocol@literalbuffered{false \gp@temp\space colorimage}%
  \pgfsysprotocol@literal{#6 >}%
}
\def\gp@rawimage@html#1#2#3#4#5#6{%
% FIXME: print a warning message here
}

\ifgppdfout
  \def\gp@rawimage{\gp@rawimage@pdf}
\else
  \ifgppsout
    \def\gp@rawimage{\gp@rawimage@ps}
  \else
    \def\gp@rawimage{\gp@rawimage@html}
  \fi
\fi


\def\gploadimage#1#2#3#4#5{%
  \pgftext[left,bottom,x=#1cm,y=#2cm] {\pgfimage[interpolate=false,width=#3cm,height=#4cm]{#5}};%
}

\def\gp@set@size#1{%
  \def\gp@image@size{#1}%
}

\def\gp@rawimage@#1#2#3#4#5#6#7#8{
  \tikz@scan@one@point\gp@set@size(#6,#7)\relax%
  \tikz@scan@one@point\pgftransformshift(#2,#3)\relax%
  \pgftext {%
    \pgfsys@beginpurepicture%
    \gp@image@size% fill \pgf@x and \pgf@y
    \gp@rawimage{#1}{#4}{#5}{\pgf@x}{\pgf@y}{#8}%
    \pgfsys@endpurepicture%
  }%
}

%% \gprawimage{color model}{xcoord}{ycoord}{# of xpixel}{# of ypixel}{xsize}{ysize}{rgb/cmyk hex data RRGGBB/CCMMYYKK ...}{file name}
%% color model is 'cmyk' or 'rgb' (default)
\def\gprawimage#1#2#3#4#5#6#7#8#9{%
  \ifx&#9&%
    \gp@rawimage@{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}
  \else
    \ifgppsout
      \gp@rawimage@{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}
    \else
      \gploadimage{#2}{#3}{#6}{#7}{#9}
    \fi
  \fi
}

%
% gnuplottex comapatibility
% (see http://www.ctan.org/tex-archive/help/Catalogue/entries/gnuplottex.html)
%

\def\gnuplottexextension@lua{\string tex}
\def\gnuplottexextension@tikz{\string tex}

%
% gnuplot variables getter and setter
%

\def\gpsetvar#1#2{%
  \expandafter\xdef\csname gp@var@#1\endcsname{#2}
}

\def\gpgetvar#1{%
  \csname gp@var@#1\endcsname %
}

%
% some wrapper code
%

% short for a filled path
\def\gpfill#1{\path[line width=0.1\gpbaselw,draw,fill,#1]}

% short for changing the line width
\def\gpsetlinewidth#1{\pgfsetlinewidth{#1\gpbaselw}}

% short for changing the line type
\def\gpsetlinetype#1{\tikzset{gp path/.style={#1,#1 add}}}

% short for changing the dash pattern
\def\gpsetdashtype#1{\tikzset{gp path/.append style={#1}}}

% short for changing the point size
\def\gpsetpointsize#1{\tikzset{gp point/.style={mark size=#1\gpbasems}}}

% wrapper for color settings
\def\gpcolor#1{\tikzset{global #1}}
\tikzset{rgb color/.code={\pgfutil@definecolor{.}{rgb}{#1}\tikzset{color=.}}}
\tikzset{global rgb color/.code={\pgfutil@definecolor{.}{rgb}{#1}\pgfutil@color{.}}}
\tikzset{global color/.code={\pgfutil@color{#1}}}

% prevent plot mark distortions due to changes in the PGF transformation matrix
% use `\gpscalepointstrue' and `\gpscalepointsfalse' for enabling and disabling
% point scaling
%
\newif\ifgpscalepoints
\tikzset{gp shift only/.style={%
  \ifgpscalepoints\else shift only\fi%
}}
\def\gppoint#1#2{%
  \path[solid] plot[only marks,gp point,mark options={gp shift only},#1] coordinates {#2};%
}


%
% char size calculation, that might be used with gnuplottex
%
% Example code (needs gnuplottex.sty):
%
%    % calculate the char size when the "gnuplot" style is used
%    \tikzset{gnuplot/.append style={execute at begin picture=\gpcalccharsize}}
%
%    \tikzset{gnuplot/.append style={font=\ttfamily\footnotesize}}
%
%    \begin{tikzpicture}[gnuplot]
%      \begin{gnuplot}[terminal=lua,%
%          terminaloptions={tikz solid nopic charsize \the\gphcharsize,\the\gpvcharsize}]
%        test
%      \end{gnuplot}
%    \end{tikzpicture}
%
%%%
% The `\gpcalccharsize' command fills the lengths \gpvcharsize and \gphcharsize with
% the values of the current default font used within nodes and is meant to be called
% within a tikzpicture environment.
% 
\newdimen\gpvcharsize
\newdimen\gphcharsize
\def\gpcalccharsize{%
  \pgfinterruptboundingbox%
  \pgfsys@begininvisible%
  \node at (0,0) {%
    \global\gphcharsize=1.05\fontcharwd\font`0%
    \global\gpvcharsize=1.05\fontcharht\font`0%
    \global\advance\gpvcharsize by 1.05\fontchardp\font`g%
  };%
  \pgfsys@endinvisible%
  \endpgfinterruptboundingbox%
}

%
%  define a rectangular node in tikz e.g. for the plot area
%
%  #1 node name
%  #2 coordinate of "south west"
%  #3 coordinate of "north east"
%
\def\gpdefrectangularnode#1#2#3{%
  \expandafter\gdef\csname pgf@sh@ns@#1\endcsname{rectangle}
  \expandafter\gdef\csname pgf@sh@np@#1\endcsname{%
    \def\southwest{#2}%
    \def\northeast{#3}%
  }
  \pgfgettransform\pgf@temp%
  % once it is defined, no more transformations will be applied, I hope
  \expandafter\xdef\csname pgf@sh@nt@#1\endcsname{\pgf@temp}%
  \expandafter\xdef\csname pgf@sh@pi@#1\endcsname{\pgfpictureid}%
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%  You may want to adapt the following to fit your needs (in your 
%%  individual style file and/or within your document).
%%

%
% style for every plot
%
\tikzset{gnuplot/.style={%
  >=stealth',%
  line cap=round,%
  line join=round,%
}}

\tikzset{gp node left/.style={anchor=mid west,yshift=-.12ex}}
\tikzset{gp node center/.style={anchor=mid,yshift=-.12ex}}
\tikzset{gp node right/.style={anchor=mid east,yshift=-.12ex}}

% basic plot mark size (points)
\newdimen\gpbasems
\gpbasems=.4pt

% basic linewidth
\newdimen\gpbaselw
\gpbaselw=.4pt

% this is the default color for pattern backgrounds
\colorlet{gpbgfillcolor}{white}

% set background color and fill color
\def\gpsetbgcolor#1{%
  \pgfutil@definecolor{gpbgfillcolor}{rgb}{#1}%
  \tikzset{tight background,background rectangle/.style={fill=gpbgfillcolor},show background rectangle}%
}

% this should reverse the normal text node presets, for the
% later referencing as described below
\tikzset{gp refnode/.style={coordinate,yshift=.12ex}}

% to add an empty label with the referenceable name "my node"
% to the plot, just add the following line to your gnuplot
% file:
%
% set label "" at 1,1 font ",gp refnode,name=my node"
%

% enlargement of the bounding box in standalone mode (only used by LaTeX/ConTeXt)
\def\gpbboxborder{0mm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%  The following TikZ-styles are derived from the 'pgf.styles.*' tables
%%  in the Lua script.
%%  To change the number of used styles you should change them there and
%%  regenerate this style file.
%%

% arrow styles settings
\tikzset{gp arrow 1/.style={>=latex}}
\tikzset{gp arrow 2/.style={>=angle 90}}
\tikzset{gp arrow 3/.style={>=angle 60}}
\tikzset{gp arrow 4/.style={>=angle 45}}
\tikzset{gp arrow 5/.style={>=o}}
\tikzset{gp arrow 6/.style={>=*}}
\tikzset{gp arrow 7/.style={>=diamond}}
\tikzset{gp arrow 8/.style={>=open diamond}}
\tikzset{gp arrow 9/.style={>={]}}}
\tikzset{gp arrow 10/.style={>={[}}}
\tikzset{gp arrow 11/.style={>=)}}
\tikzset{gp arrow 12/.style={>=(}}

% plotmark settings
\tikzset{gp mark 0/.style={mark size=.5\pgflinewidth,mark=*}}
\tikzset{gp mark 1/.style={mark=+}}
\tikzset{gp mark 2/.style={mark=x}}
\tikzset{gp mark 3/.style={mark=star}}
\tikzset{gp mark 4/.style={mark=square}}
\tikzset{gp mark 5/.style={mark=square*}}
\tikzset{gp mark 6/.style={mark=o}}
\tikzset{gp mark 7/.style={mark=*}}
\tikzset{gp mark 8/.style={mark=triangle}}
\tikzset{gp mark 9/.style={mark=triangle*}}
\tikzset{gp mark 10/.style={mark=triangle,every mark/.append style={rotate=180}}}
\tikzset{gp mark 11/.style={mark=triangle*,every mark/.append style={rotate=180}}}
\tikzset{gp mark 12/.style={mark=diamond}}
\tikzset{gp mark 13/.style={mark=diamond*}}
\tikzset{gp mark 14/.style={mark=otimes}}
\tikzset{gp mark 15/.style={mark=oplus}}

% pattern settings
\tikzset{gp pattern 0/.style={white}}
\tikzset{gp pattern 1/.style={pattern=north east lines}}
\tikzset{gp pattern 2/.style={pattern=north west lines}}
\tikzset{gp pattern 3/.style={pattern=crosshatch}}
\tikzset{gp pattern 4/.style={pattern=grid}}
\tikzset{gp pattern 5/.style={pattern=vertical lines}}
\tikzset{gp pattern 6/.style={pattern=horizontal lines}}
\tikzset{gp pattern 7/.style={pattern=dots}}
\tikzset{gp pattern 8/.style={pattern=crosshatch dots}}
\tikzset{gp pattern 9/.style={pattern=fivepointed stars}}
\tikzset{gp pattern 10/.style={pattern=sixpointed stars}}
\tikzset{gp pattern 11/.style={pattern=bricks}}

% if the 'tikzplot' option is used the corresponding lines will be smoothed by default
\tikzset{gp plot axes/.style=}
\tikzset{gp plot border/.style=}
\tikzset{gp plot 0/.style=smooth}
\tikzset{gp plot 1/.style=smooth}
\tikzset{gp plot 2/.style=smooth}
\tikzset{gp plot 3/.style=smooth}
\tikzset{gp plot 4/.style=smooth}
\tikzset{gp plot 5/.style=smooth}
\tikzset{gp plot 6/.style=smooth}
\tikzset{gp plot 7/.style=smooth}

% linestyle settings
\tikzset{gp lt axes/.style=dotted}
\tikzset{gp lt border/.style=solid}

% linestyle "addon" settings for overwriting a default linestyle within the
% TeX document via eg. \tikzset{gp lt plot 1 add/.style={fill=black,draw=none}} etc.
\tikzset{gp lt axes add/.style={}}
\tikzset{gp lt border add/.style={}}
\tikzset{gp lt plot 0 add/.style={}}
\tikzset{gp lt plot 1 add/.style={}}
\tikzset{gp lt plot 2 add/.style={}}
\tikzset{gp lt plot 3 add/.style={}}
\tikzset{gp lt plot 4 add/.style={}}
\tikzset{gp lt plot 5 add/.style={}}
\tikzset{gp lt plot 6 add/.style={}}
\tikzset{gp lt plot 7 add/.style={}}
\tikzset{gp lt plot 0/.style={}}
\tikzset{gp lt plot 1/.style={}}
\tikzset{gp lt plot 2/.style={}}
\tikzset{gp lt plot 3/.style={}}
\tikzset{gp lt plot 4/.style={}}
\tikzset{gp lt plot 5/.style={}}
\tikzset{gp lt plot 6/.style={}}
\tikzset{gp lt plot 7/.style={}}

% linestyle color settings
\colorlet{gp lt color axes}{black!30}
\colorlet{gp lt color border}{black}

% dash type settings
% Define this as a macro so that the dash patterns expand later with the current \pgflinewidth.
\def\gpdashlength{\pgflinewidth}
\tikzset{gp dt 0/.style={solid}}
\tikzset{gp dt 1/.style={solid}}
\tikzset{gp dt 2/.style={dash pattern=on 7.5*\gpdashlength off 7.5*\gpdashlength}}
\tikzset{gp dt 3/.style={dash pattern=on 3.75*\gpdashlength off 5.625*\gpdashlength}}
\tikzset{gp dt 4/.style={dash pattern=on 1*\gpdashlength off 2.8125*\gpdashlength}}
\tikzset{gp dt 5/.style={dash pattern=on 11.25*\gpdashlength off 3.75*\gpdashlength on 1*\gpdashlength off 3.75*\gpdashlength}}
\tikzset{gp dt 6/.style={dash pattern=on 5.625*\gpdashlength off 5.625*\gpdashlength on 1*\gpdashlength off 5.625*\gpdashlength}}
\tikzset{gp dt 7/.style={dash pattern=on 3.75*\gpdashlength off 3.75*\gpdashlength on 3.75*\gpdashlength off 11.25*\gpdashlength}}
\tikzset{gp dt 8/.style={dash pattern=on 1*\gpdashlength off 3.75*\gpdashlength on 11.25*\gpdashlength off 3.75*\gpdashlength on 1*\gpdashlength off 3.75*\gpdashlength}}
\tikzset{gp dt solid/.style={solid}}
\tikzset{gp dt axes/.style={dotted}}

% command for switching to colored lines
\def\gpcoloredlines{%
  \colorlet{gp lt color 0}{red}%
  \colorlet{gp lt color 1}{green}%
  \colorlet{gp lt color 2}{blue}%
  \colorlet{gp lt color 3}{magenta}%
  \colorlet{gp lt color 4}{cyan}%
  \colorlet{gp lt color 5}{yellow}%
  \colorlet{gp lt color 6}{orange}%
  \colorlet{gp lt color 7}{purple}%
}

% command for switching to monochrome (black) lines
\def\gpmonochromelines{%
  \colorlet{gp lt color 0}{black}%
  \colorlet{gp lt color 1}{black}%
  \colorlet{gp lt color 2}{black}%
  \colorlet{gp lt color 3}{black}%
  \colorlet{gp lt color 4}{black}%
  \colorlet{gp lt color 5}{black}%
  \colorlet{gp lt color 6}{black}%
  \colorlet{gp lt color 7}{black}%
}

%
% some initialisations
%
% by default all lines will be colored
\gpcoloredlines
\gpsetpointsize{4}
\gpsetlinetype{gp lt solid}
\gpscalepointsfalse
\endinput


==> gnuplot-lua-tikz.tex <==
%%
%%  plain TeX wrapper for gnuplot-tikz style file
%%
\input tikz.tex
\usetikzlibrary{arrows,patterns,plotmarks,backgrounds}

\edef\tikzatcode{\the\catcode`\@}
\catcode`\@=11

\input gnuplot-lua-tikz-common.tex


\catcode`\@=\tikzatcode

\endinput


==> t-gnuplot-lua-tikz.tex <==
%%
%%  ConTeXt wrapper for gnuplot-tikz style file
%%
\usemodule[tikz]

\usetikzlibrary[arrows,patterns,plotmarks,backgrounds]

\edef\tikzatcode{\the\catcode`\@}
\edef\tikzbarcode{\the\catcode`\|}
\edef\tikzexclaimcode{\the\catcode`\!}
\catcode`\@=11
\catcode`\|=12
\catcode`\!=12

\input gnuplot-lua-tikz-common.tex

\catcode`\@=\tikzatcode
\catcode`\|=\tikzbarcode
\catcode`\!=\tikzexclaimcode

\endinput

